Co-Located Human-Human Interaction Analysis using Nonverbal Cues: A Survey

Automated co-located human-human interaction analysis has been addressed by the use of nonverbal communication as measurable evidence of social and psychological phenomena. We survey the computing studies (since 2010) detecting phenomena related to social traits (e.g., leadership, dominance, personality traits), social roles/relations, and interaction dynamics (e.g., group cohesion, engagement, rapport). Our target is to identify the nonverbal cues and computational methodologies resulting in effective performance. This survey differs from its counterparts by involving the widest spectrum of social phenomena and interaction settings (free-standing conversations, meetings, dyads, and crowds). We also present a comprehensive summary of the related datasets and outline future research directions which are regarding the implementation of artificial intelligence, dataset curation, and privacy-preserving interaction analysis. Some major observations are: the most often used nonverbal cue, computational method, interaction environment, and sensing approach are speaking activity, support vector machines, and meetings composed of 3-4 persons equipped with microphones and cameras, respectively; multimodal features are prominently performing better; deep learning architectures showed improved performance in overall, but there exist many phenomena whose detection has never been implemented through deep models. We also identified several limitations such as the lack of scalable benchmarks, annotation reliability tests, cross-dataset experiments, and explainability analysis.

==> dataset.tex <==
\begin{table*}
\centering
\label{tableDataset}
%\begin{longtable}{p{3.4cm}p{2.5cm}p{1.6cm}p{4.5cm}p{3.9cm}}
\caption{A summary of face-to-face social interaction datasets. $S$ refers to the annotations performed by the participants to asses themselves, $E$ refers to the annotation performed by external observers and $A$ stands for the annotations obtained by applying automatic methods. The datasets are listed chronologically.}
\label{tableDataset}
\begin{tabular}{p{3.4cm}p{2.5cm}p{1.6cm}p{4.5cm}p{3.9cm}} \hline
\textbf{Dataset} & \textbf{Scenario} & \textbf{Group Size / \newline Total \newline \#Participants} & \textbf{Annotations} & \textbf{Sensors} \\ \hline
Idiap Wolf \cite{Wolf2010} & Game play (sitting participants) & 8-12/36 & Roles (E), Speaking Activity (E) & HSM, ARM, WC \\ \hline
%IMADE \cite{Yasuyuki2010} & & & & \\ \hline
Cocktail Party \cite{Zen2010} & Indoor free-standing/moving conversations & 6-7/13 & Extroversion ($S$), Neuroticism ($S$) & FFC, PTZ \\ \hline
Coffee Break \cite{Cristani2011} & Indoor free-standing/moving conversations & 6-14 & Groups ($E$) & Fish-eye camera \\ \hline
\cite{Feese2011b} & Meeting (??) & 3/126 & Behavior (e.g., face-touch, nodding) ($E$), Leadership style ($E$) & IMU \\ \hline %NOT PUB. AVAILABLE
%\cite{Hagad2011} & & & & \\ \hline %NOT PUB. AVAILABLE
\cite{Chen2011} & Daily interactions in a research lab. & 3-5/5 & Social groups ($A$), participant's location ($A$) and head orientation ($A$), & RGB cameras, RFID \\ \hline
Twenty-Question Game \cite{Kalimeri2011} & Brainstorming/problem solving meetings through a game & 4/52 & Dominance ($S$), Group performance ($E$)& SB \{Prox., ACC, microphone\} \\ \hline
\cite{Srivastava2012} & 3907 video clips from movies & 50 characters & Emotions ($A$), Personality Traits ($A$) & DMC \\ \hline
SocioMetric Badges \cite{Lepri2012b} & Monitoring the activity of people in a research institution for 6 weeks & 53 & Personality traits ($S$), affective states ($S$), Perceived productivity/relations ($S$)  & SB \{microphone, infrared beam and detector, bluetooth detector and ACC\} \\ \hline
ELEA \cite{SanchezCortes2012} & Meeting (survival task) & 3-4/148 & Personality Traits ($S$), Leadership ($S$, $E$), Competence ($S$), Likeness ($S$), Ranked Dominance ($S$) & LAM, ARM, WC  \\ \hline
First-Person Social Interaction \cite{Fathi2012} & Day-long first-person videos in a theme park & 8 & Social interaction type: dialogue, discussion, monologue, etc. ($E$), activities: walking, waiting, sitting, buying, eating, etc. ($E$) & GoPro \\ \hline
D64 \cite{Oertel2012} & Free-sitting conversations & 4-5 & Overall group excitement ($E$), pairwise social distance between participants ($E$) & HSM, LAM, OMCS \\ \hline
KTH Wolf \cite{Oertel2013} & Role-play based game (sitting participants) & 8 & Eye gaze ($E$), voice activity ($E$), group involvement ($E$) & CUC  \\ \hline
YouTube Social Roles \cite{Ramanathan2013} & YouTube videos of events (birthday party, Catholic weeding, etc.) & 964 & Event names ($E$), Social roles ($E$) & DMC \\ \hline
SONVB \cite{Nguyen2014} & Real job interviews (1 interviewer and 1 interviewee) & 62 & Hirability scores ($E$), personality traits ($S$), Intelligence ($S$), communication and persuasion skills ($S$) & ARM, CUC \\ \hline
EGO-GROUP \cite{Alletto2014} & First-person video segments in a lab., coffee break, conference room and outdoor & 13 video segments & Group identifier for each person ($E$) & Narrative camera\\ \hline
MATRICS \cite{Nihei2014} & Meeting (discussion based on roles) & 4 / 40 & Personality Traits ($S$), (not)influential statements ($E$) & OMCS, ACC, Kinect, ET, FSC, WC, HSM \\ \hline
SALSA \cite{AlamedaPineda2015} & Indoor free-standing conversations & 18 & Personality Traits ($S$), Position ($E$), Head / Body Orientation ($E$), F-formation ($A$) & FSC, SB \{microphone, infrared beam and detector, bluetooth detector and ACC\} \\ \hline
%\cite{Kumano2015} & & & & \\ \hline
KTH-Idiap Group-Interviewing \cite{Oertel2014} & Role-play group interviews (1 interviewer and 3 interviewees sitting around a round table) & 4/20 & Eye gaze ($E$), voice activity ($E$), personality traits ($S$), interest-level/performance/potential related questionnaire ($E$), performance ($E$)  & Kinect, GoPro, CTM \\ \hline
PAVIS Leadership \cite{Beyan2016} & Meeting (survival task) & 4/64 & Leadership ($S$, $E$), designate leaders ($S$), leadership style ($E$), voice activity ($E$), face-touch behavior ($E$) & LAM, CUC \\ \hline
%iTag \cite{Moreno2016}  & Game & & & \\ \hline
MobileSSI \cite{Flutura2016} & Pub (free discussions) & 3& Voice activity ($E$), laughter ($E$) & LAM, Smartphone \{ACC\}\\ \hline
\cite{Terven2016} & Meeting (sitting participants, topic-defined conversations) & 2/48 & Head nodding ($E$), conversation usefulness ($E$), sustained concentration ($E$), competence ($E$), the level of satisfaction ($E$) & Smart glasses, CUC \\ \hline
%\cite{Era2017} & & & & \\ \hline
\cite{Nanninga2017} & Meeting (??) & 3-8/107 & Cohesion ($E$) & ARM, HSM, HD cameras, ACC\\ \hline
\cite{Ohnishi2017} & Storytelling events & 14 & Interest level ($E$), observed action ($E$) & ACC, Gyro, HD camera \\ \hline
MatchNMingle \cite{MatchNMingle} & Indoor free-standing conversations and speed dates & 8-2 / 94 & Personality Traits ($S$), Self Control Scale ($S$), Sociosexual Orientation Inventory ($S$), Social Cues ($E$), Social Actions ($E$), F-formations ($E$) & Wearable devices composed of triaxial ACC and Prox., GoPro Hero, TVC. \\ \hline
MULTISIMO \cite{koutsombogera2018} & Meeting (solving a quiz) & 3 / 49 & Personality Traits ($S$, $E$), Experience ($S$), Speaking Activity ($A$), Dominance ($E$), Transcripts ($E$), Turn-taking ($A$), Emotions ($A$). & CUC, C360, HSM, ODM, Kinect. \\ \hline
AMIGOS \cite{Correa2018} & Watching videos & 4 / 20 \newline (in group setting) & Personality traits ($S$), Mood ($S$), Valence ($S$, $E$), Arousal ($S$, $E$), Dominance ($S$), Liking ($S$), Familiarity ($S$), Emotions ($S$). & Electroencephalogram (EEG), Electrocardiogram (ECG), and Galvanic Skin Response (GSR) sensors, CUC, Kinect. \\ \hline
MPIIGroupInteraction \cite{Muller2018} & Meeting (sitting participants, topic-defined conversations)  & 3-4/78 & Rapport ($E$), Leadership ($S$), Dominance ($S$), Competence ($S$), Liking ($S$), Personality Traits ($S$) & LAM, CUC, FSC, CTM \\ \hline
Focused Interaction \cite{Bano2018} & Daily-life interactions in indoor, outdoor, day\&night, office and campus & 19 sessions & (No)focused interaction ($E$), voice activity ($A$) & GoPro, ACC, GYRO, MAG, smartphone (GPS) \\ \hline
%GoPro Hero4, shoulder mounted, video and voice activity are released. Focused, unfocused ad no interaction along between persons. Continuous videos captured at various locations (indoor, outdoor, day and night, office, campus)
UGI \cite{Bhattacharya2018} & & & & \\ \hline
SRIV \cite{Jinna2018} & & & & \\ \hline
TeamSense \cite{Zhang2018} & & & & \\ \hline
Panoptic \cite{Joo2019} & Game (standing participants) & 3-12 & Roles ($E$), Speaking activity ($E$) & HD and VGA cameras, Kinect\\ \hline
%UGI \cite{Bhattacharya2019} & & & & \\ \hline
GAP \cite{Braley2018,Kubasova2019} & & & & \\ \hline
VGAF \cite{Sharma2019} & & & & \\ \hline
EgoSocialRelation \cite{Aghaei2016,Aimar2019} & & & & \\ \hline
%Aghaei2016: ego centric interaction or not an interaction annotations: narrative camera, body mounted, no audio only video, bounding boxes around faces in each video frame is given. Multiple short photo streams always containing one or more individuals at times involved in interaction with the camera wearer.-- Aimar2019: s 693 sequences, grouped in five domains and nine relations, namely Attachment (father-child, mother-child), Reciprocity (friends, classmates), Mating (lovers), Coalitional group (colleagues), and Hierarchical group (presenter-audience, leader-subordinate
\cite{Katevas2019} & & & & \\ \hline
%%%%%%%%%\endfirsthead
Video Social Relation \cite{Liu_2019_CVPR} & & & & \\ \hline
\cite{Echeverria2019} & & & & \\ \hline
Resistance Game\cite{Chongyang2019} & & & & \\ \hline
NTHULP \cite{Zhong_interspeech_2019} & & & & \\ \hline
\cite{Othman2019} & & & & \\ \hline
GAME-ON \cite{Maman2020} & Game (standing/moving participants) & 3 / 51 & Cohesion ($S$), Leadership ($S$), Emotional State ($S$), Warmth and Competences ($S$) & IMU (ACC, GYRO, MAG), infrared, RGB cameras, HSM. \\ \hline
WoNoWa \cite{Biancardi2020} & & & & \\ \hline
\cite{Girolami2020} & & & & \\ \hline
\cite{Onishi2020} & & & & \\ \hline
%\cite{Muralidhar2020} & & & & \\ \hline VIDEO INTERVIEWS: NO INTERACTION, PARTICIPANTS ONLY ANSWERS THE QUESTIONS APPEARING ON THE SCREEN
\cite{Subburaj2020} & & & & \\ \hline
\cite{Lahnakoski2020} & & & & \\ \hline
\cite{Zhang_2020_WACV} & & & & \\ \hline
\end{tabular}
\end{table*}
%%%%%%%%%\end{longtable}



%\begin{table}
%\centering
%\label{tableDataset}
%\caption{A summary of face-to-face social interaction datasets (listed chronologically) in terms of ``scenarios'', ``group size/total number of participants'', ``annotations'' and ``the sensors used'', respectively. $S$ refers to the annotations performed by the participants to assess themselves, $E$ refers to the annotation performed by external observers and $A$ stands for the annotations obtained by applying automatic methods.}
%\resizebox{!}{9cm}{
%\label{tableDataset}
%\begin{tabular}{p{14.5cm}}
% \midrule
%\textbf{Dataset} & \textbf{Scenario} & \textbf{Group Size / \newline Total \newline \#Participants} & \textbf{Annotations} & \textbf{Sensors} \\ \hline

\noindent
$\bullet$ \textbf{ Idiap Wolf \cite{Wolf2010}:} Game play (sitting participants); 8-12 / 36; roles (E), speaking activity (E); HSM, ARM, WC. \\
$\bullet$ \textbf{ Cocktail Party \cite{Zen2010}:} Indoor free-standing/moving conversations; 6-7 / 13; extroversion ($S$), neuroticism ($S$); FFC, PTZ. \\
$\bullet$ \textbf{ Coffee Break \cite{Cristani2011}:} Indoor free-standing/moving conversations; 6-14; groups ($E$); fish-eye camera. \\
$\bullet$ \textbf{ \cite{Feese2011b}:} Meeting (discussion based on roles); 3 / 126; behavior (e.g., face-touch, nodding) ($E$), leadership style ($E$); IMU. \\ %NOT PUB. AVAILABLE
%\cite{Hagad2011} ; ; ; ; \\  %NOT PUB. AVAILABLE
$\bullet$ \textbf{ \cite{Chen2011}:} Daily interactions in a research lab.; 3-5 / 5; social groups ($A$), participant's location ($A$) and head orientation ($A$); RGB cameras, RFID. \\ 
$\bullet$ \textbf{ Twenty-Question Game \cite{Kalimeri2011}:} Brainstorming/problem solving games; 4 / 52; dominance ($S$), group performance ($E$); SB (Prox., ACC, microphone). \\ 
$\bullet$ \textbf{ \cite{Srivastava2012}:} 3907 video clips from movies; 50 characters; emotions ($A$), personality traits ($A$); DMC. \\ 
$\bullet$ \textbf{ SocioMetric Badges \cite{Lepri2012b}:} Monitoring the activity of people in a research institution for 6 weeks; 53; personality traits ($S$), affective states ($S$), perceived productivity/relations ($S$); SB (microphone, infrared beam and detector, bluetooth detector and ACC). \\ 
$\bullet$ \textbf{ ELEA \cite{SanchezCortes2012}:} Meeting (survival task); 3-4 / 148; personality traits ($S$), leadership ($S$,$E$), competence ($S$), likeness ($S$), dominance ($S$); LAM, ARM, WC. \\ 
$\bullet$ \textbf{ First-Person Social Interaction \cite{Fathi2012}:} Day-long first-person videos in a theme park; 8; social interaction type: dialogue, discussion, monologue, etc. ($E$), activities: walking, waiting, sitting, buying, eating, etc. ($E$); GoPro. \\ 
$\bullet$ \textbf{ D64 \cite{Oertel2012}:} Free-sitting conversations; 4-5; overall group excitement ($E$), pairwise social distance between participants ($E$): HSM, LAM, OMCS. \\ 
$\bullet$ \textbf{ KTH Wolf \cite{Oertel2013}:} Role-play based game (sitting participants); 8; Eye gaze ($E$), voice activity ($E$), group involvement ($E$); CUC.  \\ 
$\bullet$ \textbf{ YouTube Social Roles \cite{Ramanathan2013}:} YouTube videos of events (birthday party, Catholic weeding, etc.); 964 videos; event names ($E$), social roles ($E$); DMC. \\ 
$\bullet$ \textbf{ SONVB \cite{Nguyen2014}:} Real job interviews; 3 / 62; hirability ($E$), personality traits ($S$), intelligence ($S$), communication and persuasion skills ($S$); ARM, CUC. \\ 
$\bullet$ \textbf{ EGO-GROUP \cite{Alletto2014}:} Indoor/outdoor first-person video segments; 13 video segments; group identifier for each person ($E$); narrative camera. \\ 
$\bullet$ \textbf{ MATRICS \cite{Nihei2014}:} Meeting (role-based discussions); 4 / 40; personality traits ($S$), (not)influential statements ($E$); OMCS, ACC, Kinect, ET, FSC, WC, HSM. \\ 
%\cite{Kumano2015} ; ; ; ; \\ 
$\bullet$ \textbf{ KTH-Idiap Group-Interviewing \cite{Oertel2014}:} Role-play group interviews (1 interviewer and 3 interviewees sitting around a round table); 4 / 20; eye gaze ($E$), voice activity ($E$), personality traits ($S$), interest-level/performance/potential related questionnaire ($E$), performance ($E$); Kinect, GoPro, CTM. \\ 
$\bullet$ \textbf{MAHNOB \cite{MAHNOB2015}:} Dyadic discussions and negotiations; 2 / 60; motor mimicry behavior of head gestures, hand gestures, body movement and facial expressions ($E$), reflective mimicry ($E$); CUC, HSM, far-field microphone.
\\
$\bullet$ \textbf{ SALSA \cite{AlamedaPineda2015}:} Indoor free-standing conversations (poster presentation session, cocktail party); 18; personality traits ($S$), position ($E$), head/body orientation ($E$), F-formation ($A$); FSC, SB (microphone, infrared beam and detector, bluetooth detector and ACC). \\
$\bullet$ \textbf{ PAVIS Leadership \cite{Beyan2016,Beyan2020ICMI}:} Meeting (survival task); 4 / 64; leadership ($S$, $E$), designate leaders ($S$), leadership style ($E$), voice activity ($E$), face-touching behavior ($E$); LAM, CUC. \\ 
%iTag \cite{Moreno2016}  ; Game ; ; ; \\ 
$\bullet$ \textbf{ MobileSSI \cite{Flutura2016}:} Pub (free discussions); 3; voice activity ($E$), laughter ($E$); LAM, smartphone (ACC). \\ 
$\bullet$ \textbf{ \cite{Terven2016}:} Meeting (sitting participants, topic-defined conversations); 2 / 48; head nodding ($E$), conversation usefulness ($E$), sustained concentration ($E$), competence ($E$), the level of satisfaction ($E$); smart glasses, CUC. \\ 
% not physical f2f interaction $\bullet$ \textbf{NoXi \cite{NoXi2017}:} ; ; ; ; \\ 
$\bullet$ \textbf{ \cite{Nanninga2017}:} Business meeting; 3-8 / 107; cohesion ($E$); ARM, HSM, HD cameras, ACC. \\ 
$\bullet$ \textbf{ \cite{Ohnishi2017}:} Storytelling events; 14; interest level ($E$), observed action ($E$); ACC, Gyro, HD camera. \\ 
$\bullet$ \textbf{ MatchNMingle \cite{MatchNMingle}:} Indoor free-standing conversations (cocktail party) and speed dates; 8-2 / 94; personality traits ($S$), self control scale ($S$), sociosexual orientation inventory ($S$), social cues ($E$), social cautions ($E$), F-formations ($E$); wearable devices composed of triaxial ACC and Prox., GoPro, TVC. \\ 
$\bullet$ \textbf{ MULTISIMO \cite{koutsombogera2018}:} Meeting (solving a quiz); 3 / 49; personality traits ($S$, $E$), experience ($S$), speaking activity ($A$), dominance ($E$), transcripts ($E$), turn-taking ($A$), emotions ($A$); CUC, C360, HSM, ODM, Kinect. \\ 
$\bullet$ \textbf{ AMIGOS \cite{Correa2018}:} Watching videos; 4 / 20 (in group setting); personality traits ($S$), mood ($S$), valence ($S$, $E$), arousal ($S$, $E$), dominance ($S$), liking ($S$), familiarity ($S$), emotions ($S$); electroencephalogram (EEG), electrocardiogram (ECG), and galvanic skin response (GSR) sensors, CUC, Kinect. \\ 
$\bullet$ \textbf{ MPIIGroupInteraction \cite{Muller2018}:} Meeting (sitting participants, topic-defined conversations); 3-4 / 78; rapport ($E$), leadership ($S$), dominance ($S$), competence ($S$), liking ($S$), personality traits ($S$); LAM, CUC, FSC, CTM. \\ 
$\bullet$ \textbf{ Focused Interaction \cite{Bano2018}:} Daily-life interactions in indoor, outdoor, day\&night, office and campus; 19 sessions; (No)focused interaction ($E$), voice activity ($A$); GoPro, ACC, GYRO, MAG, smartphone (GPS). \\ 
$\bullet$ \textbf{ UGI \cite{Bhattacharya2018}}: Meeting (survival tasks); 4 / 36; perceived leadership ($E$), perceived contribution ($E$) ; Time-of-Flight sensors, Kinect, LAM. \\ 
$\bullet$ \textbf{ SRIV \cite{Jinna2018}:} Movies and TV dramas; 69 movies, 3124 videos; subjective relations, e.g., dominant, competitive, trusting, warm, friendly, attached, etc. ($E$), objective relations, e.g., supervisor-subordinate, peer, parent-offspring ($E$); DMC. \\ 
$\bullet$ \textbf{ TeamSense \cite{Zhang2018}:} Four-month simulation of a space
exploration mission at a remote location; 6; roles ($E$), affective states ($S$), team cohesiveness ($S$); SB (microphone, infrared beam and detector, bluetooth detector and ACC).  \\ 
$\bullet$ \textbf{ Panoptic \cite{Joo2019}:} Game (standing participants); 3-12; roles ($E$), speaking activity ($E$); HD and VGA cameras, Kinect. \\ 
$\bullet$ \textbf{ GAP \cite{Braley2018}:} Meetings (survival task); 2-3 / 37; group satisfaction ($E$), group decision-making ($E$), dialogue acts ($E$), sentiment ($E$), transcription ($E$); WC, handy recorder. \\ 
$\bullet$ \textbf{ VGAF \cite{Sharma2019}:} Web videos containing groups; 1004 videos; group-level emotion ($E$), group-level cohesion ($E$); DMC. \\ 
$\bullet$ \textbf{ EgoSocialRelation \cite{Aghaei2016,Aimar2019}:} Daily-life indoor/outdoor situations; 8 camera wearer / 35 video sequences with 100 different people; sequence annotation ($E$), face locations ($E$),
social interaction state ($E$), social relations, e.g., father-child, lovers, friends, classmates, etc. ($E$); narrative camera. \\ 
$\bullet$ \textbf{ \cite{Katevas2019}:} Social networking event; 22; social groups ($E$) ; Smartphone (iBeacon Prox., ACC, Gravity, rotation rate), HD cameras. \\ 
$\bullet$ \textbf{ ViSR \cite{Liu_2019_CVPR}:} Movies; 8000 video clips; social relations, e.g., leaders-subordinates, colleague, friend, sibling, etc. ($E$); DMC. \\ 
$\bullet$ \textbf{ \cite{Echeverria2019}:} Patient-centred and health care simulation; 4 / 9; roles ($E$), collaboration translucence ($E$); electrodermal activity sensor, ACC, ARM, HD camera. \\ 
$\bullet$ \textbf{ Resistance Game \cite{Chongyang2019}:} Game play; 5-8 / 233; roles ($E$), dominance ($E$); HD video camera. \\ 
$\bullet$ \textbf{ NTHULP \cite{Zhong_interspeech_2019}:} Meetings (discussion based on roles); 3 / 194; roles ($E$), personality traits ($S$), group performance outcome ($E$); CUC, LAM. \\
$\bullet$ \textbf{ \cite{Othman2019}:} Game (standing participants); 4 / 96; transcriptions ($E$), text binary content parameters ($E$), group contribution ($E$), CUC, HSM. \\ 
$\bullet$ \textbf{ GAME-ON \cite{Maman2020}:} Game (standing/moving participants); 3 / 51; Cohesion ($S$), Leadership ($S$), Emotional State ($S$), Warmth and Competences ($S$); IMU (ACC, GYRO, MAG), infrared, RGB cameras, HSM. \\ 
$\bullet$ \textbf{ WoNoWa \cite{Biancardi2020}} Indoor free-standing conversations performing a pre-defined task; 3 / 45; voice activity ($A,E$), quantity of motion ($A$), head position and rotation ($A$), chronemics ($E$), proxemics ($E$), kinesics ($E$), leadership ($S$), degree of acquaintance ($S$), warmth and competence ($E$), perceived transactive memory system ($E$); HD handy camera, HSM. \\ 
%$\bullet$ \textbf{ \cite{Girolami2020}:} ; ; (no)interaction/approaching ($M$) ;Bluetooth Beacons, smartphones \\ 
$\bullet$ \textbf{ \cite{Onishi2020}:} Meeting (sitting participants, topic-defined conversations); 2 / 34; dialogue data ($E$), praising skills ($E$); CUC, HSM. \\ 
%\cite{Muralidhar2020} ; ; ; ; \\  VIDEO INTERVIEWS: NO INTERACTION, PARTICIPANTS ONLY ANSWERS THE QUESTIONS APPEARING ON THE SCREEN
%$\bullet$ \textbf{ \cite{Subburaj2020}:} ; ; ; \\ 
$\bullet$ \textbf{ \cite{Lahnakoski2020}:} Topic pre-defined conversations and cooperative / competitive game-play; 2 / 18; gaze ($E$), head location/orientation ($E$), enjoyment ($E$), choice ($E$), felt pressure ($E$), effort ($E$), personality traits ($E$); Kinect, IMU \\ 
$\bullet$ \textbf{ \cite{Zhang_2020_WACV}:} Meeting (survival task); 3-4 / 48; personality traits ($S$), contribution level ($E$), leadership ($E$); CUC, Kinect. \\ 
$\bullet$ \textbf{UDIVA \cite{Palmero_2021_WACV}:} Competitive and collaborative tasks (talk, game-play, lego building, gaze-events); 2 / 147; personality scores ($S$, $E$), sociodemographics ($S$), mood ($S$), fatigue ($S$), relationship type ($S$); LAM, CUC, ODM, egocentric CAM, wearable heart rate monitor. 
%\hline
%\end{tabular}}
%\end{table}
%%%%%%%%%\end{longtable}
